Africanus IV. The Stimela2 framework: scalable and reproducible workflows, from local to cloud compute

Stimela2 is a new-generation framework for developing data reduction workflows. It is designed for radio astronomy data but can be adapted for other data processing applications. Stimela2 aims at the middle ground between ease of development, human readability, and enabling robust, scalable and reproducible workflows. It represents workflows by linear, concise and intuitive YAML-format "recipes". Atomic data reduction tasks (binary executables, Python functions and code, and CASA tasks) are described by YAML-format "cab definitions" detailing each task's "schema" (inputs and outputs). Stimela2 provides a rich syntax for chaining tasks together, and encourages a high degree of modularity: recipes may be nested into other recipes, and configuration is cleanly separated from recipe logic. Tasks can be executed natively or in isolated environments using containerization technologies such as Apptainer. The container images are open-source and maintained through a companion package called cult-cargo. This enables the development of system-agnostic and fully reproducible workflows. Stimela2 facilitates the deployment of scalable, distributed workflows by interfacing with the Slurm scheduler and the Kubernetes API. The latter allows workflows to be readily deployed in the cloud. Previous papers in this series used Stimela2 as the underlying technology to run workflows on the AWS cloud. This paper presents an overview of Stimela2's design, architecture and use in the radio astronomy context.

==> stimela-clippings.tex <==
\begin{verbatim}
    _include: file1.yml
    # multiple files may be included like this:
    _include: [file1.yml, file2.yml]
    # or, equivalently, like this:
    _include: 
      - file1.yml
      - file2.yml
    \end{verbatim}
      
    Note that, since keys cannot be repeated, only one ``{\tt \_include}'' key per section is permitted (but it can specify multiple files). The result is that the file(s) (the \emph{includees}) are read in and parsed, and their content (which is expected to be [nested] namespaces) is \emph{merged} into the \emph{includer} section. Any further content in the includer then 
    \emph{augments} the included content -- that is, included keys may be modified, and new keys may be introduced. This is best illustrated by an example. If {\tt file1.yml} contains the following:
    
    {\small\begin{verbatim}
    a:
      x: 1
      y: 2
    \end{verbatim}}
    
    \noindent and {\tt file2.yml} contains the following:
    
    {\small\begin{verbatim}
    a:
      x: 2
      z: 4
    b:
      t: 1  
    \end{verbatim}}
    
    \noindent and the {\tt include-example.yml} then includes them as follows:
    
    {\small\begin{verbatim}
    _include: file1.yml
    a:
      x: 5
    
    bar:
      _include: 
        - file1.yml
        - file2.yml
      b:
        s: 6
      c:
        q: 7
    \end{verbatim}}
    
    \noindent then ultimately, the result of loading {\tt include-example.yml} looks like
    
    {\small\begin{verbatim}
    a:
      x: 5   # this value was augmented at top level
      y: 2   # this came from file1.yml
    bar:
      a:
        x: 2   # this came from file1.yml and was augmented by file2.yml
        y: 2   # this came from file1.yml
        z: 4   # this came from file2.yml
      b:
        t: 1   # this came from file2.yml
        s: 6   # this was augmented at top level
      c:
        q: 7   # this was augmented at top level
    \end{verbatim}}
      
    Similarly, the \emph{use} construct merges the content of one or more previously defined sections into the current section. It is invoked via a ``\_use'' key in the given section, with the names of the section(s) to be merged in, in dotted format. For example, if the file ``{\tt use-example.yml}'' contains
    
    {\small\begin{verbatim}
    _include: include-example.yml
    
    baz:
      _use: 
        - bar.a
        - bar.b 
      z: 10
    \end{verbatim}}
    
    \noindent then the result of loading it will look as follows:
    
    {\small\begin{verbatim}
    a:
      # (content of 'a' as per above)
    bar:
      # (content of 'bar' as per above)
    baz:
      x: 2   # this came from bar.a
      y: 2   # this came from bar.a
      z: 10  # this was augmented by baz
      t: 1   # this came from bar.b
      s: 6   # this came from bar.b
    \end{verbatim}}
      
    The example above also illustrates that includes (and uses) can be chained, and that use-constructs can refer to included content. 
    
    Use- and include-constructs are the lynchpins of modularity in \stimela\ recipes and configurations. Fundamentally, they allow for snippets of YAML to be defined in one place and reused in other places, library-style. As a real-life illustration, consider the case of CASA tasks. \stimela\ provides cab definitions for many CASA tasks, allowing them to be invoked individually from any step of the recipe. A number of these tasks (particularly, those that operate on visibility data) share a common collection of parameters which are used to specify the input measurement set, and a data selection to be performed on that measurement set. Rather than repetitively listing these parameters within each cab's schema (which would be laborious and error-prone), we list this collection of parameters once in a ``library'' file called ``casa.yml``: 
    
    {\small\begin{verbatim}
    lib:
      params:
        casa:
          mssel_inputs:  # a standard section for CASA tasks that have a vis argument, and a standard set of data selection options
            ms:
              info: "Name of input visibility file"
              dtype: MS
              writable: true
              required: true
              nom_de_guerre: vis
            field:
              info: "Select field using field id(s) or field name(s)"
              dtype: str
            spw:
              info: "Select spectral window/channels"
              dtype: str
            intent:
              info: Select observing intent
              dtype: str
          #  ...
    \end{verbatim}}
    
    We can then reuse this library content within any CASA task cab definition:
    
    {\small\begin{verbatim}
    _include: casa.yml
    
    cabs:
      casa.applycal:
        inputs:
          # pull in standard set of MS selection parameters
          _use: lib.params.casa.mssel_inputs
          # and now define some task-specific paramaters:
          docallib:
            info: "Use callib or traditional cal apply parameters"
            dtype: bool
          # ...
    \end{verbatim}}
    
    Other applications of this are libraries of recipes, and even step templates.
    
